A new wake-merging method for wind-farm power prediction in presence of heterogeneous background velocity fields

Many wind farms are placed near coastal regions or in proximity of orographic obstacles. The meso-scale gradients that develop in these zones make wind farms operating in velocity fields that are rarely uniform. However, all existing wake-merging methods in engineering wind-farm wake models assume a homogeneous background velocity field in and around the farm, relying on a single wind-speed value usually measured several hundreds of meters upstream of the first row of turbines. In this study, we derive a new momentum-conserving wake-merging method capable of superimposing the waked flow on a heterogeneous background velocity field. We couple the proposed wake-merging method with four different wake models, i.e. the Gaussian, super-Gaussian, double-Gaussian and Ishihara model, and we test its performance against LES data, dual-Doppler radar measurements and SCADA data from the Horns Rev, London Array, and Westermost Rough farm. Next to this, as an additional point of reference, the standard Jensen model with quadratic superposition is also included. Results show that the new method performs similarly to linear superposition of velocity deficits in homogeneous conditions but it shows better performance when a spatially varying background velocity is used. The most accurate estimates are obtained when the wake-merging method is coupled with the double-Gaussian and Gaussian single-wake model. The Ishihara model also shows good agreements with observations. In contrast to this, the Jensen and super-Gaussian wake model underestimate the farm power output for all wind speeds, wind directions and wind farms considered in our analysis.

==> Makefile <==
## Makefile
## Copyright 2011 Mohamed El Morabity
#
# This work may be distributed and/or modified under the conditions of the LaTeX
# Project Public License, either version 1.3 of this license or (at your option)
# any later version. The latest version of this license is in
# http://www.latex-project.org/lppl.txt and version 1.3 or later is part of all
# distributions of LaTeX version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Mohamed El Morabity
#
# This work consists of all files listed in manifest.txt.

######################
# Fonts informations #
######################

FONT_NAME = lato
FOUNDRY = public
FONT_CODES = fla

# Supported LaTeX encodings
SUPPORTED_ENCODINGS = ot1 t1 ts1
# Supported LaTeX encodings containing small caps
SUPPORTED_SC_ENCODINGS = $(filter-out ts1,$(SUPPORTED_ENCODINGS))
# Custom encodings provided
INPUT_ENCODINGS = $(INPUT_ETX_FILES:$(FONT_NAME)-%.etx=%)


#####################
# Installation root #
#####################

TEXMFHOME = $(shell kpsexpand '$$TEXMFHOME')


###########
# Archive #
###########

ARCHIVE_ROOT = $(FONT_NAME)
ARCHIVE = $(FONT_NAME).zip


###########
# Sources #
###########

TRUETYPE_FILES = $(wildcard *.ttf)

# Fontinst files
FONTINST_FILE = $(FONT_NAME)-drv.tex
FONTINST_MAP_FILE = $(FONT_NAME)-map.tex

# Custom Fontinst encoding files
INPUT_ETX_FILES = $(FONT_NAME)-01.etx $(FONT_NAME)-02.etx $(FONT_NAME)-dotlessj.etx
MTX_FILES = $(FONT_NAME)-fixlatin.mtx $(FONT_NAME)-fixtextcomp.mtx

STYLE_FILES = $(wildcard *.sty)

DOCUMENTATION = $(FONT_NAME).tex $(FONT_NAME).pdf $(FONT_NAME)-samples.tex $(FONT_NAME)-samples.pdf README CHANGES

# Files to be installed in texmf/source
SOURCE_FILES = $(FONTINST_FILE) $(FONTINST_MAP_FILE) $(INPUT_ETX_FILES) $(MTX_FILES) Makefile ttf2type1.pe


###################
# Generated files #
###################

TYPE1_FILES = $(TRUETYPE_FILES:.ttf=.pfb) $(TRUETYPE_FILES:.ttf=-LCDFJ.pfb)
AFM_FILES = $(TYPE1_FILES:.pfb=.afm)

# Fontinst log file
FONTINST_REC_FILE = $(FONT_NAME)-rec.tex

# Metrics files
PL_FILES = $(foreach e,$(INPUT_ENCODINGS),   \
             $(TRUETYPE_FILES:.ttf=-$(e).pl) \
           )
OUTPUT_MTX_FILES = $(PL_FILES:.pl=.mtx)
VPL_FILES = $(foreach e,$(SUPPORTED_ENCODINGS),          \
              $(TRUETYPE_FILES:.ttf=-$(e).vpl)           \
            )                                            \
            $(foreach e,$(SUPPORTED_SC_ENCODINGS),       \
              $(TRUETYPE_FILES:.ttf=-SmallCaps-$(e).vpl) \
            )
TFM_FILES = $(PL_FILES:.pl=.tfm) $(VPL_FILES:.vpl=.tfm)
VF_FILES = $(VPL_FILES:.vpl=.vf)

MAP = $(FONT_NAME).map

# Font definition files
FD_FILES = $(foreach e,$(SUPPORTED_ENCODINGS), \
             $(foreach f,$(FONT_CODES),        \
               $(e)$(f).fd                     \
             )                                 \
           )

# Generated encoding files
ENC_FILES = $(INPUT_ETX_FILES:.etx=.enc)

# Generated files to be installed
GENERATED_FILES = $(TYPE1_FILES) $(AFM_FILES) $(TFM_FILES) $(VF_FILES) $(MAP) $(FD_FILES) $(ENC_FILES)


default: all


all: dist


dist: $(ARCHIVE)


%.pfb %.afm: %.ttf
	fontforge ttf2type1.pe $<
	# BUGFIX: fix FontName to the name of the file
	sed -i "s/^FontName .*/FontName $*/" $*.afm


%-LCDFJ.pfb: %.pfb
	t1dotlessj $< $@


%-LCDFJ.afm: %-LCDFJ.pfb
	pf2afm $<
	# BUGFIX: fix FontName to the name of the file
	sed -i "s/^FontName .*/FontName $*/" $*.afm


%.tfm: %.pl
	pltotf $< $@


%.tfm: %.vpl
	vptovf $^ $


%.vf: %.vpl
	vptovf $^ $@


$(FONTINST_REC_FILE): $(AFM_FILES) $(MTX_FILES) $(FONTINST_FILE)
	latex $(FONTINST_FILE)


$(PL_FILES) $(VPL_FILES): $(FONTINST_REC_FILE)


$(MAP): $(FONTINST_REC_FILE) $(FONTINST_MAP_FILE)
	latex $(FONTINST_MAP_FILE)


$(FD_FILES) $(ENC_FILES): $(MAP)


texmf-tree: clean-texmf-tree $(GENERATED_FILES) $(SOURCES_FILES)
	mkdir -p $(ARCHIVE_ROOT)/doc/fonts/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/tex/latex/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/fonts/{enc,map}/dvips/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/fonts/{afm,tfm,truetype,type1,vf}/$(FOUNDRY)/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/source/fonts/$(FONT_NAME)/
	cp -p $(DOCUMENTATION) $(ARCHIVE_ROOT)/doc/fonts/$(FONT_NAME)/
	cp -p $(FD_FILES) $(STYLE_FILES) $(ARCHIVE_ROOT)/tex/latex/$(FONT_NAME)/
	cp -p $(ENC_FILES) $(ARCHIVE_ROOT)/fonts/enc/dvips/$(FONT_NAME)/
	cp -p $(MAP) $(ARCHIVE_ROOT)/fonts/map/dvips/$(FONT_NAME)/
	cp -p $(AFM_FILES) $(ARCHIVE_ROOT)/fonts/afm/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TFM_FILES) $(ARCHIVE_ROOT)/fonts/tfm/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TRUETYPE_FILES) $(ARCHIVE_ROOT)/fonts/truetype/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TYPE1_FILES) $(ARCHIVE_ROOT)/fonts/type1/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(VF_FILES) $(ARCHIVE_ROOT)/fonts/vf/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(SOURCE_FILES) $(ARCHIVE_ROOT)/source/fonts/$(FONT_NAME)/
	cp -p README $(ARCHIVE_ROOT)
	cd $(ARCHIVE_ROOT) && find . -type f > manifest.txt


$(ARCHIVE): clean-texmf-tree texmf-tree
	zip -r $@ $(ARCHIVE_ROOT)


install: texmf-tree
	mkdir -p $(TEXMFHOME)
	cp -a $(ARCHIVE_ROOT)/* $(TEXMFHOME)
	texhash
	updmap --enable Map=$(MAP)


uninstall:
	$(RM) -r $(TEXMFHOME)/doc/latex/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/tex/latex/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/fonts/{enc,map}/dvips/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/fonts/{afm,tfm,type1,vf}/$(FOUNDRY)/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/source/$(FONT_NAME)/
	updmap --disable $(MAP)
	texhash


clean: clean-texmf-tree
	$(RM) $(TYPE1_FILES) $(AFM_FILES)
	$(RM) $(FONTINST_REC_FILE)
	$(RM) $(PL_FILES) $(TYPE1_FILES:.pfb=.pl)
	$(RM) $(OUTPUT_MTX_FILES) $(TYPE1_FILES:.pfb=.mtx)
	$(RM) $(VPL_FILES)
	$(RM) $(TFM_FILES)
	$(RM) $(VF_FILES)
	$(RM) $(MAP)
	$(RM) $(FD_FILES)
	$(RM) $(ENC_FILES)
	$(RM) $(ARCHIVE)
	$(RM) *~ *.log


clean-texmf-tree:
	$(RM) -r $(ARCHIVE_ROOT)


.PHONY: clean clean-texmf-tree texmf-tree

